Preech: A System for Privacy-Preserving Speech Transcription

New Advances in machine learning have made Automated Speech Recognition (ASR) systems practical and more scalable. These systems, however, pose serious privacy threats as speech is a rich source of sensitive acoustic and textual information. Although offline and open-source ASR eliminates the privacy risks, its transcription performance is inferior to that of cloud-based ASR systems, especially for real-world use cases. In this paper, we propose Pr$\epsilon\epsilon$ch, an end-to-end speech transcription system which lies at an intermediate point in the privacy-utility spectrum. It protects the acoustic features of the speakers' voices and protects the privacy of the textual content at an improved performance relative to offline ASR. Additionally, Pr$\epsilon\epsilon$ch provides several control knobs to allow customizable utility-usability-privacy trade-off. It relies on cloud-based services to transcribe a speech file after applying a series of privacy-preserving operations on the user's side. We perform a comprehensive evaluation of Pr$\epsilon\epsilon$ch, using diverse real-world datasets, that demonstrates its effectiveness. Pr$\epsilon\epsilon$ch provides transcriptions at a 2% to 32.25% (mean 17.34%) relative improvement in word error rate over Deep Speech, while fully obfuscating the speakers' voice biometrics and allowing only a differentially private view of the textual content.

==> abstract_for_hotcrp.tex <==

New advances in machine learning and the abundance of speech datasets have made Automated Speech Recognition (ASR) systems, with very high accuracy, a reality.   ASR systems offer their users the means to transcribe speech data at scale.  Unfortunately, these systems pose serious privacy threats as speech is a rich source of sensitive acoustic and textual information. 
Although offline ASR eliminates the privacy risks, we find that its transcription performance is inferior to that of cloud-based ASR systems, especially for real-world recordings. In this paper, we propose Pr$\epsilon\epsilon$ch, an end-to-end speech transcription system which lies at an intermediate point in the privacy-utility spectrum of speech transcription. It protects the acoustic features of the speakers’ voices and protects the privacy of the textual content at an improved performance relative to offline ASR. Pr$\epsilon\epsilon$ch relies on cloud-based services to transcribe a speech file after applying a series of privacy-preserving operations on the user’s side. We perform a comprehensive evaluation of Pr$\epsilon\epsilon$ch, using diverse real-world datasets, that demonstrates its effectiveness. Pr$\epsilon\epsilon$ch provides transcriptions at a 12.30%


New advances in machine learning have made Automated Speech Recognition (ASR) systems practical. ASR systems can transcribe speech data at scale.  Unfortunately, these systems pose serious privacy threats as speech is a rich source of sensitive acoustic and textual information. 
Although offline ASR eliminates the privacy risks, its transcription performance is inferior to that of cloud-based ASR systems, especially for real-world use cases. In this paper, we propose Pr$\epsilon\epsilon$ch, an end-to-end speech transcription system which lies at an intermediate point in the privacy-utility spectrum of speech transcription. It protects the acoustic features of the speakers’ voices and protects the privacy of the textual content at an improved performance relative to offline ASR. Additionally, Pr$\epsilon\epsilon$ch provides several control knobs to allow customizable utility-usability-privacy trade-off. It relies on cloud-based services to transcribe a speech file after applying a series of privacy-preserving operations on the user’s side. We perform a comprehensive evaluation of Pr$\epsilon\epsilon$ch, using diverse real-world datasets, that demonstrates its effectiveness. Pr$\epsilon\epsilon$ch provides transcriptions at a 2%



==> eval_Copy.tex <==

\section{Implementation and Evaluation}
\label{sec:impl_eval}
In this section, we describe the implementation specifics of \name along with its evaluation.

\subsection{Implementation}
\label{sec:implementaton}
\input{5_3_Implementation.tex}

\subsection{Evaluation}
\label{sec:evaluation}
We evaluate how well \name meets the design objectives of Sec.~\ref{sec:OurSys} at the different states of the trade-off control knobs. In particular, we aim to answer the following questions: (\textit{Q1.}) Does \name preserve the transcription utility? (\textit{Q2.}) Does \name protect the voice biometrics of the speakers? (\textit{Q3.}) Does \name protect the textual content of the speech at the \CSP's side?  (\textit{Q4.}) Does the different control knobs  provide  substantial flexibility in the utility-usability-privacy spectrum? %

We answer the first three questions with respect to a prototype implementation of \name that provides the maximum degree of privacy and hence least utility.  While evaluating \textit{Q4}, we relax the privacy guarantee to obtain utility and usability improvements.

\textbf{Prototype} \name: The prototype is 
\begin{enumerate} \item segmentation algorithm to ensure contains at most two non-stop words \item dummy text is generated from  \item May-to-one voice conversion for \item  \end{enumerate}
\subsubsection{Q1. Transcription Utility} \label{sec:transcriptionUtility}



\begin{table*}[t]
\begin{minipage}[c]{0.60\linewidth}\centering
\scalebox{0.9}{
\begin{tabular}{@{}lcccccc@{}}\toprule
\textbf{Datasets} & \textbf{Cloning} & \textbf{KWS} & \textbf{One-to-One} & \textbf{Many-to-One} & \textbf{Deep Speech}\\ 
\midrule
VCTK p266 & 5.15 & -- & 16.55  & 21.92(17.96\%) & 26.72\\
VCTK p262 & 4.53 & -- & 7.39 & 10.82(32.25) & 15.97\\
\midrule
Facebook1 & 5.76 & 8.26 & 11.39 & 19.66(20.47) & 24.72\\
Facebook2 & 8.63 & 9.75 & 17.19 & 19.15(28.03) & 26.61\\
Facebook3 & 8.20 & 14.93 & 21.27 & 23.75(22.69) & 30.72\\
\midrule
Carpenter1 & 9.44 & 14.43 & 22.92 & 20.43(20.97) & 25.85\\
Carpenter2 & 9.22 & 13.53 & 32.47 & 36.30(8.59) & 39.71\\
\bottomrule
\end{tabular}}
\caption{WER (\%) at different options of \name privacy levels \rev{change colns titles}}
\label{tab:WER_VC_4levels}
\end{minipage}
\begin{minipage}[c]{0.4\linewidth}
\centering
\includegraphics[width=0.85\textwidth]{figures/KWS/KWS_limited.png}
\captionof{figure}{Sensitive keywords detection curve: TPR vs FPR at different values of the sensitivity score.}
\label{fig:KWS}
\end{minipage}
\end{table*}




We assess the transcription \WER after deploying \name on the non-standard datasets.
Table~\ref{tab:WER_noVC} in Sec.~\ref{sec:utility_privacy} shows the \WER of the \CSPs before applying \name to the employed datasets. It shows the baseline performance of the \CSPs and \OSPs for speech transcription. 

\paragraph{\WER Analysis:}
Column five in Table~\ref{tab:WER_VC_4levels} shows \WER for the prototype \name that employs the final  many-to-one voice conversion. There are two main observations -- first, many-to-one \VC is superior to  Deep Speech. Specifically, \name's relative improvement over Deep Speech ranges from 8.59\% to 32.25\% over the evaluation datasets which is a significant result with reference to current \ASR literature~\cite{park2019specaugment, chan2016listen, hannun2014deep}. Second,  \name does not have the same performance for all the datasets. This observation arises again from the lack of diversity in our training set. For example, if we break down the Carpenter set by speaker (Carpenter 1 and Carpenter 2), the speaker in Carpenter 1 speaks loudly and clearly allowing our \VC system to perform well. On the other hand, the second speaker (Carpenter 2) is not as clear or loud, which results in an inferior \VC performance. This finding is consistent across the \CSPs and Deep Speech as well. Our experiments show that these results can be improved by adding samples of the same speaker to the training pipeline of $net1$ and $net2$. We chose not to go with this approach (or report these results) as this limits the usability of the system and in such case sprocket would be a better choice. 

\WER for each dataset at each design option of \name.
There are three takeaways from the table. First, the \WER suffers quite a bit due to applying many-to-one voice conversion; the \WER drops to 10-36\% compared to 5-10\% in the base case \CSP's performance. %
Recall that we trained the \VC system before applying \name using standard \ASR corpora, while we evaluate the \WER on non-standard cases. Still, \name's \WER is superior to that of Deep Speech, which has been trained through hundreds of hours of speech data. \name's improvement over Deep Speech ranges from 8.59\% to 32.25\% over the evaluation datasets which is indeed a significant result with reference to current \ASR literature~\cite{park2019specaugment, chan2016listen, hannun2014deep}. 


Second, sprocket significantly outperforms the many-to-one \VC. This result is expected since sprocket is trained and tested on the same subset of source speakers while the many-to-one \VC system generalizes to previously unseen speakers. These findings highlight the \textit{trade-off} between usability and utility: if a user has access to representative samples of a source speaker, they can use them to improve the performance of \name.


Third, \name does not have the same performance for all the datasets. This observation arises again from the lack of diversity in our training set. For example, if we break down the Carpenter set by speaker (Carpenter 1 and Carpenter 2), the speaker in Carpenter 1 speaks loudly and clearly allowing our \VC system to perform well. On the other hand, the second speaker (Carpenter 2) is not as clear or loud, which results in an inferior \VC performance. This finding is consistent across the \CSPs and Deep Speech as well. Our experiments show that these results can be improved by adding samples of the same speaker to the training pipeline of $net1$ and $net2$. We chose not to go with this approach (or report these results) as this limits the usability of the system and in such case sprocket would be a better choice. 




\subsubsection{Q2. Voice Biometric Privacy}
\label{sec:ident_diariz_exp}


By design, the many-to-one \VC system (Sec.~\ref{sec:VoiceConversion}) removes all the identifying features from the speech file, including the speakers' voices, background noise and recording hardware. On the other hand, the one-to-one \VC system translates the acoustic features from a source to a target speaker voice. Hence, it may leak some features from the source speaker. To test and validate these properties, we conduct two experiments using the voice analysis APIs from a \CSP.

In the first experiment, we assess the \CSP's ability to separate speech belonging to different speakers after \name applies the \VC systems. In our multi-speaker datasets, IBM diarization API detects only one speaker . Note that The DER of the IBM API was very low before applying \VC as is evident from the results in Table~\ref{tab:diar_results} on the same datasets. Furthermore, we run the converted voice samples after adding the dummy segments (after \TTS and \VC) through IBM's diarization API. Again, the API detects only one speaker. Thus, not only does \name hide the speakers biometrics and map them to a single target speaker but also ensures noise indistinguishability, which is key to its privacy properties. 



The second experiment tests \name's privacy properties against a stronger adversary, who has access to samples for the true speakers. We enroll segments from the true speakers as well as the fake target speaker to Azure's Speaker Identification API from Microsoft. We pass the segments from \name (after adding dummy segments and applying \VC) to the API. 
When many-to-one \VC is applied, in all cases the API identifies the segments as belonging to the fake target speaker. Not a single segment was matched to the original speaker. Both experiments show that through many-to-one \VC, \name is effective in sanitizing the speakers voice and ensuring noise indistinguishability. 
When one-to-one \VC is applied, on average 10\% of the segments were identified to their true speakers. This result again highlights the trade-off between utility and privacy. The user can choose a privacy level that is a bit vulnerable against a stronger attacker in order to maintain high transcription accuracy (utility).






\subsubsection{Q3. Sensitive Words Scrubbing}

We run PocketSphinx keyword spotting on each dataset at different sensitivity scores ranging from 0.2 to 1. Fig.~\ref{fig:KWS} shows the detection True Positive Rate (TPR) versus the False Positive Rate (FPR), also called the false-alarm rate, at different sensitivity scores. As the figure shows, at any TPR, the sensitivity score can be tuned to minimized the false-alarm rate. Thus, it enables the user to control and optimize the utility-privacy trade-off. 

Next, we evaluate the impact of sensitive words scrubbing on the transcription utility. We set a sensitivity score of 0.95 for all the datasets as to have a near perfect TPR. Our experiments show that the total duration of the segments flagged with sensitive keywords at this score is less than 20\% of the total duration of each dataset. Specifically, the duration ratios are (0.13, 0.06, 0.18, 0.20, and 0.08) for the five Facebook and Carpenter datasets. Then, we transcribe the sensitive-flagged segments using Deep Speech. The overall transcription accuracy after sensitive keywords scrubbing is presented in table~\ref{tab:WER_VC_4levels}. Since the segments are very short, the portion of speech transcribed locally is limited. Hence, the impact of \OSP transcription errors on the utility is not significant. %


\subsubsection{Q4. Textual Privacy}\label{sec:eval:text}
\name follows the DP mechanism described in Sec.~\ref{sec:DPmechanism} to obfuscate the textual content in speech. We evaluate the privacy properties of \name in two scenarios: in-vocabulary noise and extended-vocabulary noise. In the first scenario, we only consider adding dummy segments that correspond to words from the same vocabulary, $\mathcal{V}$, as that of the input speech file; we obtain the vocabulary using offline transcription as discussed in Sec.~\ref{sec:topicModel}. The second scenario considers an extended vocabulary which covers, in addition to words in $\mathcal{V}$, a random set of words from a standard English dictionary. Our text-based evaluation considers the following aspects:

\squishlist
\itemsep-0.3em 
    \item validating that the domain can be accurately estimated from offline transcription;
    \item analyzing the histogram distance between the original and noisy transcripts as a function of the distance parameters;
    \item measuring the impact of the added noise on the performance of state-of-the-art NLP APIs from Google and AWS: topic modeling, category classification, and sentiment analysis.
\squishend


\paragraph{Vocabulary Estimation:}
We estimate the vocabulary (domain) using the combined offline transcription of Deep Speech and PocketSphinx. Let $\mathcal{W}$ represent the set of unique words in $T^g_S$. We define the accuracy of the vocabulary estimation, $D_{acc}$, as the ratio between the unique count of the correctly identified words and the unique count of the words in the ground truth transcript, $|\mathcal{W}|$. For our datasets, the domain estimation accuracy equals to $75.54\%$. We also calculate the weighted estimation accuracy defined as:
$
D_{weighted} = \frac{\sum{P(w_{est}).\mathbbm{1}_{w_{est} \in \mathcal{W}}}}{|\mathcal{W}|}
$ where $P(w_{est})$ is the weight of word $w_{est}$ in the true document. $D_{weighted}$ is more informative since it gives higher weights to the most frequent words and less weight to the distribution-tail words. The weighted estimation accuracy is $99.989\%$ in our datasets. From the estimated $|\mathcal{W}|_{est}$ we select $|\mathcal{V}|$ over which we apply the DP mechanism.   

The choice of the vocabulary highlights another \textit{trade-off} between the cost and privacy in \name. Using extended-vocabulary for noise addition leads to better privacy (as is illustrated later) but results in costlier noise injection. %



\paragraph{Histogram Distance:}


\begin{table*}[t]
\small
\centering
\scalebox{1.0}{\begin{tabular}{@{}lcrcccccc@{}}\toprule
\multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{$|\mathcal{V}|$}} & {\multirow{2}{*}{\textbf{\# words}}} & \multicolumn{6}{c}{\textbf{Noise Size}}\\
 & & & \multicolumn{2}{c}{\textbf{d=2}} & \multicolumn{2}{c}{\textbf{d=5}} & \multicolumn{2}{c}{\textbf{d=15}}\\ 
\midrule
VCTK p266 & 483 & 922 (\$0.22) & 2915 & \$0.68 & 7247 & \$1.69 & 23899 & \$5.58 \\
VCTK p262& 471 & 914 (\$0.213)  & 2845 & \$0.66 & 7157 & \$1.67 & 23230 & \$5.42\\
Facebook & 1098 & 5326 (\$1.24) & 6660 & \$1.55 & 16567 & \$3.87 & 54038 & \$12.62\\
Carpenter & 1474 & 7703 (\$1.80) & 8915 & \$2.08 & 22296 & \$5.20 & 72907 & \$17.02\\
\bottomrule
\end{tabular}}
\caption{Noise size and monetary cost with varying $d$ at fixed $\epsilon=1$ and $\delta=0.05$.}
\label{tab:noise_cost}
\end{table*}


We analyze the distance between the original and noisy histograms (after applying \name) and its impact on the cost of online transcription. Because of the nature of \name's DP mechanism, the noise addition depends on four values only: $|\mathcal{V}|$, $\epsilon$, $\delta$, and $d$. 

\rev{cost = \#noise words/2.57*0.0006, where 2.57 is the TTS speaking rate, 0.0006 is the Google's cost per sec.}

For all our experiments, we fix the values of $\epsilon=1$ and $\delta=0.05$. Fig.~\ref{fig:Histogram_L1distance} shows the cost in USD for adding the noise for different values of $|\mathcal{V}|$ and $d$. The values of $|\mathcal{V}|$ are determined from our evaluation datasets. The noise cost is proportional to the number of words injected through dummy segments, the $\ell_1$ distance between the original and noisy histograms. In \name, adding more noise comes at an increased monetary cost, instead of a utility loss. 

Fig.~\ref{fig:Histogram_L1distance} highlights the \textit{trade-off} between the  privacy level and the cost of adding noise. The increase in the size of vocabulary requires adding more dummy segments to maintain the same privacy level. We also consider the case of adding extended-vocabulary noise ($|\mathcal{V}|$=2500), where the privacy gains come at an additional cost of \$25 (using both AWS and Google).







\begin{figure*}[t]     
\centering
\begin{subfigure}{0.24\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/Distance/8_topics.png}
  \caption{8 topics}
  \label{fig:cloud_1} 
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/Distance/10_topics.png}
  \caption{10 topics}
  \label{fig:cloud_2} 
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/Distance/12_topics.png}
  \caption{12 topics}
  \label{fig:cloud_3} 
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/Distance/14_topics.png}
  \caption{14 topics}
  \label{fig:cloud_4} 
\end{subfigure}
\caption{Topics $\ell_1$ distance \CDF at $d$ = 2, 5, and 15 for $t=$ 8, 10, 12, and 14}
\label{fig:topic_distance}
\end{figure*}

\paragraph{Topic Model:}
We generate the topic models from the documents corresponding to the original and noisy word histograms, and evaluate their $\ell_1$ distance. The topic model extraction operates on a corpus of documents; hence we included 8 more Supreme Court cases to our original evaluation datasets (Facebook Hearing and Carpenter case). The selected cases vary in the document size and the vocabulary size (Fig.~\ref{fig:Histogram_L1distance}). In this evaluation, we treat all of these documents as one corpus; our objective is to evaluate topic modeling after applying \name to the whole corpus.

We use AWS Comprehend API to generate the topic model. The API needs the number of topics as a hyperparameter that ranges from 1 to 100. Based on our apriori knowledge of the true number of topics, we evaluate the topic model on the following number of topics $t = 8, 10, 12, $ and $14$.

We statistically evaluate the $\ell_1$ distance between the true and noisy topics. The topic model $\mathcal{T}=\{\mathbb{T}_1,\cdots,\mathbb{T}_t\}$ is a set of $t$ topics where each $\mathbb{T}_i, i \in [t]$ is a word distribution. We use the Hungarian algorithm \cite{Hungarian} to match each noisy topic $\mathbb{T}'_i \in \mathcal{T}'$ to its closest match in $\mathcal{T}$, the true topic model. We evaluate the topics $\ell_1$ distance for 21 runs. For each run we generate the random noise vector per document, select the corresponding dummy segments, and evaluate the topic model on the set of original and noisy documents.
Fig.~\ref{fig:topic_distance} shows the empirical \CDF of the topics $\ell_1$ distance at different values of $d$. As the figure shows, the higher the distance parameter $d$, the larger is the $\ell_1$ distance between true and noisy topics.
Note that Fig.~\ref{fig:topic_distance} values represent an under-estimate of the actual distance. AWS API returns as a maximum 10 words per topic, and we assume that the other vocabulary words have zero weight in the topic. Hence, for any true-noisy topic pair we only count the distance between 20 words as a max which is not the actual case. Counting all the vocabulary words results in distances that are larger than the presented values.

\paragraph{Stylometry:}


 




\paragraph{Category Classification:} 
Document classification is a NLP task that identifies the main genre of a text document. 
Google's API can classify a document to a predefined list of 700+ document categories\footnote{https://cloud.google.com/natural-language/docs/categories}. We, first, run the classification API over the original documents from the same topic modeling corpus. All of them classify as \textsf{Law \& Government}\xspace. Running the API on \name processed documents, using an extended-vocabulary, dropped the classification accuracy to $0\%$. None of the documents got identified as any category close to legal, law, or government in this case even at the smallest value of the distance parameter chosen for our experiments ($d=2$). %
Although a portion of the noise words belongs to the original  \textsf{Law \& Government}\xspace category, segmentation, shuffling and the out-of-vocabulary words successfully confuse the \CSP's classifier.

\begin{figure}
    \centering
  \includegraphics[width=\columnwidth]{figures/Distance/Heatmap.pdf}
    \caption{Heatmap of the sentiment score of 10 documents at $d$ = 2, 5, and 15 with $\epsilon=1$ and $\delta=0.05$. $d=0$ corresponds to the original documents score}
    \label{fig:heatmap}
\end{figure}

\paragraph{Sentiment Analysis:}
Sentiment analysis generates a score ranging between $[-1, 1]$ which reflects the attitude in the text as positive, negative, or neutral. 
First, we evaluate the sentiment scores of the original 10 documents. Doc 8,9 refer to the Carpenter and Facebook Hearing cases, while Doc 0-7 refer to the other Supreme Court cases added for the topic model evaluations.
For all of them, the score falls between $-0.2$ and $-0.9$ which is expected as they represent legal documents. Next, we evaluate the scores from \name processed documents considering an extended-vocabulary. We find that all scores increase towards a more positive opinion.  Fig.~\ref{fig:heatmap} shows a heat-map of the sentiment scores as we change the distance parameter $d$ for the set of 10 evaluation documents. Thus \name's two-pronged approach -- 1) addition of extended-vocabulary noise 2) removal of ordering information via segmentation and shuffling, proves to be effective. 

In a setting where the adversary has no apriori knowledge about the general domain of our speech, the noise addition mechanism gains extend from DP guarantee over the histogram to other NLP analysis as well.



\subsubsection{\rev{Textual Analysis}}
 
Similar to our evaluations of the voice biometrics (sec.~\ref{sec:ident_diariz_exp}), we take one step further to validate \name's privacy guarantees. We exploit the state-of-the-art NLP models available to the adversary at the moment to break the textual privacy. Aside from the sensitive keywords scrubbing, the textual content privacy guarantee is based on noise addition and indistinguishibility. We perform three experiments to test the indistinguishibility of the dummy and true segments in terms of the language similarity.  


\paragraph{Most Probable Next Segment:}
In this experiment, we give the adversary the advantage of knowing a true segment $S_t$ that is at least a few sentences long from the Facebook hearing dataset. Also, we assume the user will send all the shuffled true and dummy segments to one \CSP without partitioning. We use the state-of-the-art $GPT$ language model to determine the most probable next segment following the true segment $S_t$. \rev{Define what is the perplexity score?} We get the perplexity score of stitching $S_t$ to each of the other segments. The segment with the lowest perplexity score is selected as the most probable next segment. We iterate over all the true segments of the Facebook dataset selecting them as $S_t$. 35.48\% of the time a true segment was selected as the most probable next segment and 64.52\% a dummy segment was selected. Hence, the true and dummy segments are almost equally likely in terms of their language model. This result shows that the language model could not differentiate between the true and dummy segments even when part of the true text is known to the adversary.

Next, we attempt to re-order the segments also based on the language model perplexity score. We give the adversary the advantage of knowing the first segment $S_0$. We get the perplexity score of $S_0$ followed by each of the other segments. The segment with the lowest score is selected as the second segment and so on. We use the normalized Kendall tau rank distance as a metric to measure the sortness of the segments. The normalized kendall tau distance measures the number of ...., where 0 distance means the list is perfectly sorted and 1 means the list is reversed in order. The kendall tau score of running this experiment on the Facebook dataset is 0.512. This score means the list is randomly shuffled and $GPT$ model could not re-order the segments.  



These heuristic measures show that it is hard to re-order or distinguish between the true and dummy segments. This result is expected since:
\begin{itemize}
    \item The segments are very short.
    \item The true and dummy segments follow a similar language model.
    \item We observed that most of the transcription errors happen in the first and last words of a segment due to breaking the context. These errors add to the difficulty of re-ordering.
\end{itemize}
Moreover, if the user enables partitioning between different \CSP's, no two consecutive segments goes to the same \CSP. Thus, it would be impossible to re-order the segments.




\subsubsection{Q4:}
Voice cloning reuslt in no 
\subsubsection{\rev{Usability}}
Latency
Cost maybe!
correlated histogram words?
voice conversion technique - one-to-one usability overhead
check the reviewers' comments

==> extra.tex <==
\scalebox{0.98}{\begin{tabular}{@{}lccccc@{}}\toprule
\multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{$|\mathcal{V}|$}} & {\multirow{1}{*}{\textbf{\# words}}} & \multicolumn{3}{c}{\textbf{\#Extra words due to dummy segments}}\\
 & & in $T^g_S$ & \textbf{d=2} & \textbf{d=5} & \textbf{d=15}\\ 
\midrule
VCTK p266 & 483 & 922 (\$0.22) & 2915 (\$0.68) & 7247 (\$1.69) & 23899 (\$5.58) \\
VCTK p262& 471 & 914 (\$0.21)  & 2845 (\$0.66) & 7157 (\$1.67) & 23230 (\$5.42)\\
Facebook & 1098 & 5326 (\$1.24) & 6660 (\$1.55) & 16567 (\$3.87) & 54038 (\$12.62)\\
Carpenter & 1474 & 7703 (\$1.80) & 8915 (\$2.08) & 22296 (\$5.20) & 72907 (\$17.02)\\
\bottomrule
\end{tabular}}
\caption{Noise size and monetary cost in USD with varying $d$, at $\epsilon=1$ and $\delta=0.05$.}
\label{tab:noise_cost}

==> revisionletter.tex <==
\section{Revision Letter}
We would like to thank the reviewers for their detailed and thoughtful comments, which have helped us significantly revise our paper in terms of completeness and readability. We have \textcolor{blue}{highlighted all new text in the main paper} for ease of reference.  Section 1 outlines the main changes to the paper %
while in Section 2, we address each reviewer's comment individually.
\subsection{Summary of Changes}
We denote the first comment as mentioned in Review A as RAC1 and so on.
The reviewer comments that are addressed by each of the itemized changes are stated inside the corresponding parenthesis. All the references in the revision letter to sections, figures, and tables refer to the revised submission.

\begin{itemize}\item \textbf{Clarified the user model (RAC3, RDC2, REC1):} We have included all the details of our target use case in Sec.~\ref{sec:user-system-model}. Specifically, we have clarified that \name is not designed for real-time-transcription or smart speakers applications.  \item \textbf{Clarified the threat model (RAC3, RCC1) :} We have included an end-to-end threat analysis of \name discussing its limitation in Sec.\ref{sec:ThreatModel}. We also formalise the privacy guarantee of \name. \item \textbf{Provided control knobs (RDC3):} We have heavily revised the paper to introduce \textit{control knobs} at each of the major operations of \name, namely segmentation, dummy segment generation, sensitive word scrubbing and voice conversion (Secs.~\ref{sec:Segmentation}, ~\ref{sec:DP:control_knobs}, ~\ref{sec:sws}, ~\ref{sec:VC:control_knobs},~\ref{sec:Q4}). These knobs allow the user to have a customized adaptation of \name based on their utility, usability, and privacy preferences. \item \textbf{Added a discussion on usability including latency results (RDC2, REC1):}  We have added all the necessary details on usability in our evaluation in Sec.~\ref{sec:utility_usability} and Sec.~\ref{sec:usability_privacy}. Specifically, we have added the latency results of \name in Sec.~\ref{sec:usability_privacy}. \item \textbf{Clarified the novelty of \name's use of \DP (RBC1):} We have explicitly stated the challenges and novelty of \name's use of \DP in Sec.~\ref{sec:DPnovelty}. \item \textbf{Added details on sensitive word scrubbing (RBC2, REC2):}  We have included a detailed discussion on how \name performs sensitive word scrubbing in Sec.~\ref{sec:sws}. We evaluate the efficacy of this in Sec.~\ref{sec:eval:sws}. %
\item \textbf{Included stylometry analysis (RAC4):}  
We have added stylometry analysis in our discussion on textual privacy threats (Sec.\ref{sec:textAnalysis}). The evaluations are presented in Sec.~\ref{sec:eval:text}.
\item \textbf{Included words with high \TFIDF (RAC1, RCC1c):}  We have included words with high \TFIDF in our vocabulary considered for \DP guarantee (Sec.~\ref{sec:DP:discussion}). \item \textbf{Changed dummy segment generation methodology (RCC3, REC3):} In the revised submission, dummy segments are generated from a dummy corpus automatically generated by an \NLP language model (Sec.~\ref{sec:DP:discussion}). \item \textbf{Corrected representation of \name's performance (RCC2, RDC1, REC4):} We note that the transcription accuracy results presented in the previous submission are a very conservative representation of \name's performance. We address this in the revised submission in Sec.~\ref{sec:evaluation}.
\item \textbf{Increased readability:} We have restructured the paper to increase readability keeping in mind the clarifications asked by the reviewers. \end{itemize}


\subsection{Reviewer comments}
When directly quoting reviewers comments, we will be using \textit{italic type font}. First we address the meta reviews followed by the individual comments from each reviewer.
\subsubsection{Meta-Review}
\textit{1. The privacy model / threat model that is not well defined. The paper should formalize the privacy guarantees and study the limits of the proposed solution (see reviews A, B, C for suggestions).}\\\\
We clarify the system and threat model of \name in Sec.~\ref{sec:user-system-model} and Sec.~\ref{sec:utility_privacy}. We provide a detailed end-to-end threat analysis for \name in Sec.~\ref{sec:ThreatModel}. Specifically, we discuss the limitations of \name and formalize our privacy guarantee. We address the specific comments of Review A, B, and C separately later in this section. 
\\\\
\textit{2. The discussion of the system and its evaluation are missing details and experiments, such as the impact on time overhead or usability (see reviews B, D, E for details).}\\\\
 We have added all the necessary details on usability in our evaluation in Sec.~\ref{sec:Q4_utility_privacy} and Sec.~\ref{sec:usability_privacy}. %
 \\
A point we want to highlight here is that \name is not designed for real-time transcription (Sec.~\ref{sec:user-system-model}). Specifically, examples of paradigmatic users of \name are  journalists with recordings  of confidential interviews, therapists with recordings of patients therapy sessions, and course instructors with oral examination records of students. Use cases like voice assistants and online transcription (e.g. a live-streaming press conference) are \textit{out-of-scope}. Thus, for our target use cases, latency of transcription is not a critical concern. Nevertheless we evaluate \name's latency in Sec.~\ref{sec:usability_privacy}. 
 \\
 Additionally, we have revised \name's design to improve usability. For example, dummy segments are generated from a corpus that is automatically generated by an \NLP language model (Sec.~\ref{sec:DP:discussion} and Sec.~\ref{sec:implementaton})\\
 We address the specific comments of Review B, C, and D separately later in this section. \\\\
\textit{3. Any performance improvement that diminishes the accuracy cost of privacy, or trade-off knob that enables higher accuracy at the cost of some privacy (e.g. at the level of voice conversion), would go a long way towards improving the paper}\\\\
We have heavily revised our paper (Secs.~\ref{sec:Segmentation}, ~\ref{sec:DP:control_knobs}, \ref{sec:sws}, \ref{sec:VC:control_knobs},~\ref{sec:Q4}) to introduce \textit{control knobs} at each of the major operations of \name, namely segmentation, dummy segment generation, sensitive word scrubbing and voice conversion. These knobs allow the user to have a customized adaptation of \name based on their utility, usability, and privacy preferences.  For example, if the user is not concerned  about voice privacy, then they can use the voice cloning option for transforming the dummy segments (Sec.~\ref{sec:DP:discussion}) which gives a 44\% to 80\% relative improvement in \WER over Deep Speech (Table.~\ref{tab:WER_VC_4levels}). %
Similarly, one-to-one voice conversion results in 7.6\% to 53.7\% relative improvement in \WER over Deep Speech at a weaker voice privacy level than many-to-one voice conversion (Sec.~\ref{sec:VoiceConversion}, Sec.~\ref{sec:utility_usability}, Sec.~\ref{sec:Q4_utility_privacy}). %
We evaluate the flexibility of these control knobs in  Sec.~\ref{sec:Q4}.  

\subsection{Review A:}
\textit{1. The textual analysis aims at confounding the most frequently used words, but doesn't appear to address identifiability based on the long tail: speaker or topic identification from the infrequently used words (or by the words in this corpus used more frequently than baseline). }\\\\
The rationale for protecting the most frequently used words is that most of the statistical analysis techniques (like topic modeling and stylometry analysis) are based on them.
However, if some of the distribution-tail words are deemed to be sensitive, this might indeed be a weakness. Although our empirical evaluation shows that the \OSP has a very high accuracy for the weighted estimation of the vocabulary (Sec.~\ref{sec:DPAnalysis}), some of the
 sensitive distribution-tail words might still be missed due to the transcription error of the \OSP. This is discussed in Sec.~\ref{sec:ThreatModel} in the revised paper. Nevertheless, we provide the following options to mitigate this problem:
\squishlistnum
\item  Our empirical evaluation of the tail of the word distribution showed that most of the tail words are proper nouns: names, locations, dates, etc. \name already removes them from speech file $S$ in the  sensitive word scrubbing (Sec.~\ref{sec:sws}) step.
\item In addition to the set of most frequent words, \name identifies the words with high \TFIDF (term frequency-inverse document frequency) value from the offline transcript and adds them to the vocabulary $\mathcal{V}$ considered for the \DP guarantee (Sec.~\ref{sec:DP:discussion}).  
\item The vocabulary size is a usability-privacy trade-off knob. In the extreme case, the user can include all the words in $S$ (discovered from the offline transcript) in $\mathcal{V}$. $\mathcal{V}$ can also be extended by adding out-domain-words (random words from the English dictionary - Sec.~\ref{sec:DP:discussion}). 
\squishendnum  
\textit{2. Beyond the identification of individuals from voices and the capture of specific "sensitive information" from transcripts are broader concerns with creating a permanent record of ephemeral utterances, potentially discoverable evidence contradicting white lies or changing viewpoints. What about allied concerns of surveillance capitalism, that a provider gains utility from access to aggregate data, even if non-identifying. }\\\\
\name addresses the \CSP’s data storage and analysis concerns by injecting indistinguishable dummy speech segments that allows only a differentially private view of the word histogram (and any other statistical model built over it). Hence, it introduces uncertainty and plausible deniability in the aggregated data. 
\\\\
\textit{ 3. Clarify the privacy threat model. It might be easier to understand the threat model with a paradigmatic user. Does the paper envision an interviewer, with consent, recording notes and sending them for transcription? an automated assistant parsing speech for commands? If some of the potential privacy concerns described above are out of scope, state that explicitly (and justify).} 
\\\\
We explicitly state our system and threat model in Sec.~\ref{sec:user-system-model}. Specifically, examples  of  paradigmatic  users  of \name are  journalists with recordings  of confidential interviews, therapists  with recordings of patients therapy sessions, and course instructors with oral examination  records of students. We provide a detailed end-to-end threat analysis for \name in Sec.~\ref{sec:ThreatModel}. 
\\\\
\textit{4. For textual analysis, consider the stylometry literature for adversarial model.}
\\\\
We have added stylometry analysis to the statistical analysis toolkit of the adversary (Sec.~\ref{sec:textAnalysis}). The evaluations are presented in Sec.~\ref{sec:eval:text}.


\subsubsection{Review B}

 \textit{ 1. Adopting an existing DP mechanism is incremental. The paper uses existing DP mechanism to protect textual privacy. It’s not clear what the challenges are to apply DP in this scenario.  It’s not clear what the challenges are to apply DP in this scenario. Maybe the author can elaborate more the novelty to design DP scheme for the translation scenario.}\\\\
 We discuss the challenges and the novelty of \name's use of DP in detail in Sec.~\ref{sec:DPnovelty}.\\\\
  \textit{ 2. The definition and evaluation of textual privacy are unclear. The author claims that textual privacy falls into two categories: (a). Identifying specific words from the transcript that corresponds to highly sensitive information; (b). analyzing the entire transcript on the whole with the goal of extracting some semantic information (e.g., topic modeling, category classification, and sentiment analysis). I totally agree with the first category. However, no detailed evaluation of the first category is elaborated. To be more specific, no experiments illustrate the effect of sensitive word scrubbing. If the author can design such experiments to evaluate how the proposed system can protect highly sensitive information, it would be more very impressive. As for the second point, I think the text mining tasks could be still considered as the utility task rather the private one.}\\\\
  We have included a detailed discussion on how \name performs sensitive word scrubbing in Sec.~\ref{sec:sws}. We evaluate the efficacy of this in Sec.~\ref{sec:eval:sws}. 
  \par Text mining when performed by the user, over the final transcript  obtained from \name, is a utility task. However, text mining when performed by the \CSP, over the transcript it has access to (mixed with dummy segments in \name), can be viewed as a privacy threat. Hence, we empirically evaluate \name's defense against such statistical analysis in Sec.~\ref{sec:eval:text}.\\\\
\textit{3.a. Some details of the experiment are missing. In the Abstract the authors mention ``12.30\% to 32.24\% improvement in word error rate over Deep Speech". However, No dataset information is mentioned here. It is unclear which dataset the improvement comes from.}
\\\\
The relative \WER improvement range is across all the evaluation datasets. We added the relative improvement value per dataset in Table.~\ref{tab:WER_VC_4levels}.  
\\\\
\textit{3.b. The segmentation algorithm needs a formal algorithm section to clarity it better rather than state it as plain text. }\\\\
We added a formal segmentation algorithm (Alg. 1) in the full paper \cite{FP}.
\\\\
\textit{3.c. Details of the Voice Biometric Privacy experiment is not enough. The author states that "one speaker is detected". However, it is unclear that which dataset the speaker comes from. There are just very few people in some datasets (e.g., 10 people). 10\% (1 out of 10) is still a considerable proportion.}
\\\\
In this experiment, we evaluate the cloud’s diarization API’s ability to distinguish different speakers.  Diarization does not identify a particular speaker; it only groups speech belonging to the same speaker. Hence, one speaker here means that the API could not detect that the speech is originating from multiple speakers. This result reflects the efficiency of the voice conversion system that maps both the true and dummy speech to a single target speaker voice -- the only speaker detected by the diarization API. 
\\\\
\textit{3.d. What is the noise cost (\$) in Fig. 6?}\\\\
We have replaced the figure in question with Table ~\ref{tab:noise_cost}. The table shows the number of words in the ground truth transcript, the number of extra words due to the dummy segments and the additional cost (in USD) incurred for transcribing them via the \CSP. The dummy segments are synthesized into speech using \TTS and sent to the \CSP after being shuffled with the original speech segments (steps 4, 6, and 7 in Fig.~\ref{fig:high-level}). We used Google's Speech-to-Text pricing model to get the transcription cost: \$0.009 / 15 seconds.   


\subsubsection{Review C}

\textit{1. The paper needs an in depth threat model discussion that clearly spells out the limits of the work and all the way the privacy preserving part can fail. My main complaint is that the paper lacks a very clear threat discussion that highlights the assumptions and shortcomings of the approach.} \\\\ 
We clarify the system and threat models of \name in Sec.~\ref{sec:user-system-model}. We provide a detailed end-to-end threat analysis for \name in Sec.~\ref{sec:ThreatModel}. Specifically, we discuss the limitations of \name and formalize our privacy guarantee. 
\\\\
\textit{1.a. If the attacker finds a way to reconstruct ordering, a lot of the defense collapses (and there doesn't seem to be strong arguments that they couldn't).}\\\\
If the attacker is able to re-order the segments then it will compromise our DP guarantee and thus, allow easier statistical analysis.\\ We empirically evaluate \name's resilience against re-ordering using the state-of-the-art \NLP techniques (Sec.~\ref{sec:indistinguishability_Dummy}). Our empirical results show that the adversary fails to re-order the segments in \name. However, we agree that the extent of such robustness is based on the efficacy of the  state-of-the-art \NLP techniques and hence, it is difficult to make any formal argument. We include all of this discussion in Sec.~\ref{sec:ThreatModel}. 
\\\\
\textit{1.b.  Words in a document are correlated, which typically makes DP much weaker. Here you use multiple words to measure distance, which mitigates this a bit, but for large documents would probably not be enough (or would be at a very high d and high cost).}
\\\\
Indeed, word correlations can weaken the DP guarantee ($d-w$ if $w$ is the maximum size of word groups with high correlation). This can be addressed by either increasing $d$ or considering $n$-gram $(n=w)$ word histograms. However, we agree that this would increase the requisite amount of dummy segments. We include this discussion in Sec.~\ref{sec:ThreatModel}.
\\\\
\textit{1.c. The DP guarantee only holds over the top-k words, which is pretty weak (rare words are more likely to be privacy sensitive).}
\\\\ 
Please refer to our response to Comment 1 for Review A.
\\\\
\textit{1.d. If the filtering step makes mistake, any part that is sent is leaked to the cloud provider.}
\\\\
The filtering operation has two steps: (1) identifying the list of sensitive keywords, and (2) detecting and scrubbing them from the speech segments.
The best case scenario from a privacy point of view is to have the user spell out the entire sensitive word list. However, due to its high usability overhead, \name uses \NER instead to identify proper nouns and other entities automatically from the offline transcript $T^{OSP}_S$. \name augments them with any other user-defined sensitive words.\\
In Sec.~\ref{sec:eval:sws}, we empirically show that, by tuning the sensitivity score, \name is able to achieve near perfect true positive rate (\TPR) in identifying the segments containing sensitive words (details in Sec~\ref{sec:sws}, \ref{sec:eval:sws}). However, this is a dataset dependent evaluation. 
We include this discussion in Sec.~\ref{sec:ThreatModel}.
\\\\
\textit{1.e. The topic model attack is strange: the attacker probably already has a topic model, and just wants to know the topics inside doc $D_i$. If the attacker knows about the DP mechanism, it seems like a strong attack could be designed, requiring a huge d (scaling in the number of words in the document) to prevent.}\\\\ Thm.~\ref{thm:post} guarantees that any post-processing operation on the output of a $(\epsilon,\delta)$-\DP algorithm still upholds the same \DP guarantee (even under the assumption that the DP mechanism is public). Hence, any analysis performed by an adversary on the word histogram, $\tilde{H}$ will be ``indistinguishable'' from one performed on any histogram at a distance $d$ from the original histogram $H$ (Thm.~\ref{thm:DP:topicModeling}). Thus, we show in Sec.\ref{sec:eval:statisticalAnalysis} (Fig.~\ref{fig:topic_distance}) that the noisy topic model $\mathcal{T}'=\{\mathbb{T}'_1,\cdots,\mathbb{T}'_t\}$ constructed over the noisy transcripts is significantly different from the true topic model $\mathcal{T}$ (obtained over the ground truth transcript $T^g_S$). Hence, the topics $\mathbb{T}'_i, i \in [t]$ contained in the noisy transcripts will also be significantly different from the true topics $\mathbb{T}_i, i \in [t]$.
\\ Our discussion in Sec.~\ref{sec:DP:discussion} regarding  the distance parameter $d$ and topic modeling is aimed to serve as a guide for the user in setting the value of the privacy parameters. We use topic model as our representative statistical analysis because it is one of the most natural and common place analysis that treats a document as a bag-of-words ~\cite{steyvers2007probabilistic, Ramage:2009:LLS:1699510.1699543}. However, the user is free to choose $d$ depending on the target statistical analysis the text needs protection from. %
\\\\
\textit{2. The final performance is much closer to the local model and the cloud ones, which is not a very strong performance. }\\\\
The \WER results presented in the previous submission of the paper were a very conservative evaluation of \name's transcription accuracy. Specifically, we were employing two \CSPs (based on our discussion in Sec.~\ref{sec:DP:discussion}) for the evaluation of the prototype \name. Since AWS has worse performance than Google's transcription service (Table~\ref{tab:WER_noVC}), we observed that the over all (mean) \WER was lower than that of just using Google, and did not give significant improvement over Deep Speech. However, observe that the choice of the number of \CSPs to deploy is a control knob for  the utility-usability trade-off (Sec.~\ref{sec:utility_usability}). Specifically, using multiple \CSPs  lowers  the  amount of dummy  segments  required (and hence, the monetary cost) in \name (Sec.~\ref{sec:DP:discussion}). However, as explained above, this comes at the price of utility because the transcription accuracy of the different available \CSPs vary. Note that having multiple \CSPs does not affect the formal privacy guarantee of \name. Hence, in this revised submission we present the \WER results for the prototype \name that achieves the maximum degree of formal privacy and uses only a single \CSP from Google (Table~\ref{tab:WER_VC_4levels}). We see that, \name shows 11.91\% to 32.25\% improvement in \WER over that of Deep Speech except for one dataset (Carpenter2). For the Carpenter2 dataset, the relative improvement is 2.04\%. This is so because the speaker in the dataset is not loud and clear which results in inferior voice conversion performance (Sec.~\ref{sec:transcriptionUtility}).\par Additionally, in this revised submission, we have included a discussion on various control knobs that can be tuned to obtain higher utility at the cost of usability and privacy (Secs.~\ref{sec:Q4_utility_privacy}, ~\ref{sec:usability_privacy}). For example, if the user is not concerned  about voice privacy, then (s)he can use the voice cloning option for transforming the dummy segments (Sec.~\ref{sec:DP:discussion}) that gives a 44\% to 80\% relative improvement in \WER over Deep Speech (Table.~\ref{tab:WER_VC_4levels}).  Similarly, one-to-one \VC results in 7.62\% to 53.73\% relative improvement over Deep Speech at a weaker voice privacy level than many-to-one \VC (Secs.~\ref{sec:VoiceConversion}, ~\ref{sec:utility_usability}, ~\ref{sec:Q4_utility_privacy}). %
\\\
\textit{3. It seems like the noise document require a transcription (to add the words drawn by the DP mechanism). It would be nice to state that, and explain why it isn't a problem.}\\\\
The noise \textit{text corpus} is first automatically generated in the text domain using an \NLP language model. Then, the dummy segments drawn from the DP mechanism are synthesized to speech using \TTS or voice cloning.

\subsection{Review D}
\textit{1. Results are not significantly improved over using local TTS solution.\\ My main concern with this paper is that, after all of the effort a user 
would expand to ensure privacy, the results are not significantly different
from using Deep Speech locally. Even in the best case results (Facebook 2),
given the amount of effort required to ensure privacy, I'm not convinced 
that a user would prefer the authors' approach to that of Deep Speech.}\\\\
 Please, refer to our response for Comment 2 in Review C. \\\\
\textit{2. No discussion on the performance overhead in terms of time. }\\\\
As discussed in Sec.~\ref{sec:user-system-model}, \name is not designed for real-time transcription. Specifically, examples of paradigmatic users of \name are a journalist with recordings  of confidential interviews, a therapist with recordings of patients therapy sessions, and a course instructor with oral examination records of students in an academic setting. Use cases like voice assistants and online transcription (e.g. alive-streaming press conference) are \textit{out-of-scope}. Thus, for our target use cases, latency of transcription is not a critical concern. Nevertheless we evaluate \name's latency in Sec.~\ref{sec:usability_privacy}. \\\\
\textit{3. No discussion on the privacy trade-offs available to a user (e.g., can they tweak the voice conversion so that it does not degrade the results as much, even if this sacrifices some privacy?) \\  I wonder if the authors would be open to reframing 
their paper.  It seems that, with current technology, maintaining privacy comes at a particular cost in terms of \WER (that is reasonably consistent 
between the authors' approach and using \TTS locally).  Thus what are the 
trade-offs that a user can make in terms of privacy in order to achieve 
better \WER?  Can the authors develop a set of guidelines that would help
users determine if they can reduce \WER at an acceptable loss of privacy,
or if they should accept a higher \WER knowing they have complete privacy?}
\\\\
We have heavily revised our paper (Secs.~\ref{sec:Segmentation}, ~\ref{sec:DP:control_knobs}, \ref{sec:sws}, \ref{sec:VC:control_knobs},~\ref{sec:Q4}) to introduce \textit{control knobs} at each of the major operations of \name, namely segmentation, dummy segment generation, sensitive word scrubbing and voice conversion. These knobs allow the user to have a customized adaptation of \name based on their utility, usability, and privacy preferences.  For example, if the user is not concerned  about voice privacy, then (s)he can use the voice cloning option for transforming the dummy segments (Sec.~\ref{sec:DP:discussion}) that gives a 44\% to 80\% relative improvement in \WER over Deep Speech (Table.~\ref{tab:WER_VC_4levels}). This is a 36\% to 76\% relative improvement over many-to-one \VC (perfect voice privacy) in \name. Additionally, using voice cloning shows a  $\sim 3.8 \times$ reduction in the per-segment latency over many-to-one \VC .   Similarly, one-to-one \VC results in 7.6\% to 53.7\% relative improvement over Deep Speech (6\% to 28\% over many-to-one \VC in all but one dataset) at a weaker voice privacy level than many-to-one \VC (Sec.~\ref{sec:VoiceConversion}, Sec.~\ref{sec:utility_usability}, Sec.~\ref{sec:Q4_utility_privacy}). 
 
\subsection{Review E}
\textit{1. From a performance standpoint, is Preech suitable for near
real-time transcription?  It seems very unlikely, given the costs of
some of the transformations involved and the assumptions about the
availability of related non-public datasets.  I was also disappointed
that the paper omits a performance evaluation of the Preech framework:
how long does all of this processing take?}\\\\
As discussed in Sec.~\ref{sec:user-system-model}, \name is not designed for real-time transcription. Specifically, examples of paradigmatic users of \name are a journalist with recordings  of confidential interviews, a therapist with recordings of patients therapy sessions, and a course instructor with oral examination records of students in an academic setting. Use cases like voice assistants and online transcription (e.g. alive-streaming press conference) are \textit{out-of-scope}. Thus, for our target use cases, latency of transcription is not a critical concern. Nevertheless we evaluate \name's latency in Sec.~\ref{sec:usability_privacy}.
\\\\\textit{2. \name assumes a very knowledgeable user who is capable of defining
  sensitive keywords.  Even if the user were capable of doing this,
  this seems like a very arduous undertaking, especially for large
  documents, where any proper name (for example) could be considered a
  sensitive keyword.
}\\\\
\name assumes two types of sensitive words:\\
\squishlistnum
\item named-entities like proper nouns, numbers 
\item user specified keywords
\squishendnum
For the first category, \name uses the technique of named-entity recognition (\NER) to automatically identify the set of named-entities from the offline transcript. \NER is an  information extraction technique that seeks to locate and classify named entities in text into pre-defined categories such as the names of persons, organizations, locations, expressions of times, quantities, monetary values, percentages, etc.  \\
The rationale behind the second category is to allow customization of the sensitive keyword list as users have subjective ideas of what they might consider sensitive. This discussion in included in Sec.~\ref{sec:sws}. 
Moreover, sensitive keywords scrubbing could be extended to detect words of similar semantic meaning to the user-defined list.
For example, for the Carpenter datasets  which correspond to the United States Supreme Court case concerning the privacy of historical cellphone location records, a user might consider words related to ``cellphone'' to be sensitive. However, it might be tedious to manually list down all such words. Hence, one possibility is to ask the users to provide just some \textit{seed} keywords (``cellphone'' in this context). The list of all the semantically related words can then be constructed by embedding the seed word in a vector space model and then considering all the words inside the $r$- radius ball around the seed word in the embedding space as sensitive words. The rationale behind this is that, words that have close semantic meaning will be located close to each other in the embedding space. Thus, in \name a user is expected to provide only a small, optional list of seed keywords. 
\\\\
\textit{ 3. Similarly, the requirement that there be available corpora of
  non-public documents with similar vocabularies strikes me as a very
  limiting factor for Preech.  I agree that there may be some
  particular settings where this is feasible, but I'm not convinced
  that this is generally the case.
  }
  \\\\
  We solve this problem in the revised submission by using a \NLP language model to automatically generate the dummy text corpus for \name (Sec.~\ref{sec:DP:discussion} and Sec.~\ref{sec:implementaton}). An example of the \NLP generated text is provided in the full paper \cite{FP}. %
\\\\
\textit{4. My takeaway from the Table (Table. 3) is that for perfect
privacy (Deep Speech), you get nearly comparable accuracy as \name
but can perform near real-time speech recognition and don't share any
of \name's usability problems (e.g., identifying sensitive words,
etc.).  This is my most significant concern with this paper, and is
the main reason why I lean negative.}
\\\\
Please refer to our response for Comment 2 in Review C. %
\\\\
\textit{5. As a minor editorial comment, I was surprised to see the privacy
threats enumerated in Section 3.3 and not earlier.  This seems like
good motivating material.  I recommend moving some of this into the
introduction.  That said, I thought it was a nice addition that the
authors performed actual privacy attacks (e.g., voice analysis,
speaker identification, and speaker cloning) and reported strong
results rather than merely conjecture or assert that these are
important threats.}
\\\\
We have revised the introduction (Sec.~\ref{sec:intro}) to reflect this.
\\\\
\textit{6. Why is Figure 6 presented in terms of cost (in USD)?  Can you provide
the raw number of transcripts required?  I don't quite understand what
the cost is relative to.  Is this cost per transcription?  Per
document?  Per corpus?}\\\\
We have replaced the figure in question with Table ~\ref{tab:noise_cost}. The table shows the number of words in the ground truth transcript, the number of extra words due to the dummy segments and the additional cost (in USD) incurred for transcribing them for each of the evaluation datasets. %
We used Google's Speech-to-Text pricing model to get the transcription cost: \$0.009 / 15 seconds.

